Are Children Fully Aware of Online Privacy Risks and How Can We Improve Their Coping Ability?

The age of children adopting digital technologies, such as tablets or smartphones, is increasingly young. However, children under 11 are often regarded as too young to comprehend the concept of online privacy. Limited research studies have focused on children of this age group. In the summer of 2018, we conducted 12 focus group studies with 29 children aged 6-10 from Oxfordshire primary schools. Our research has shown that children have a good understanding of certain privacy risks, such as information oversharing or avoiding revealing real identities online. They could use a range of descriptions to articulate the risks and describe their risk coping strategies. However, at the same time, we identified that children had less awareness concerning other risks, such as online tracking or game promotions. Inspired by Vygotsky's Zone of Proximal Development (ZPD), this study has identified critical knowledge gaps in children's understanding of online privacy, and several directions for future education and technology development. We call for attention to the needs of raising children's awareness and understanding of risks related to online recommendations and data tracking, which are becoming ever more prevalent in the games and content children encounter. We also call for attention to children's use of language to describe risks, which may be appropriate but not necessarily indicate a full understanding of the threats.

==> background.tex <==
\section{Background}

\subsection{Children's Perception of Privacy}

Privacy has been described as a ``concept in disarray''\cite{solove2008understanding} reflecting the complex and often overlapping conceptualisations. O'Hara proposed ``seven veils'' of privacy, spanning the conceptual, factual, phenomenological, preferential, societal, legal, and moral~\cite{ohara2016seven}. Practical research in privacy has typically spanned multiple such veils; Livingstone suggests that privacy is related to the keeping of information out of the public domain or the effective determination of \emph{what} personal information is made available to \emph{whom}~\cite{livingstone2006children}. Nissenbaum's theory of Contextual Integrity (CI) frames privacy as  ``the right to appropriate flow of personal information"~\cite{nissenbaum2004privacy} where what is ``appropriate'' is based on particular contexts and relationships.  CI has been found to be a useful practical framework to interpret people's perceptions of privacy~\cite{barkhuus2012mismeasurement,kummer2016private}.

Managing privacy is becoming increasingly challenging, and children are particularly susceptible in part due to them having little sense of the risks posed by the accumulation of personal data over time~\cite{Pangrazio:2017:MDM:3097286.3097338}. \comm{The combination of such a lack of understanding, with incentives put in place by apps and platforms to get people to share their data, have yielded the so-called `privacy paradox', a behaviour studied in teenagers~\cite{brandimarte2013misplaced} and adults~\cite{barth2017privacy} alike, in which individuals act in ways contrary to their stated privacy preferences and concerns~\cite{jones2009us,Jia:2015:RLP:2675133.2675287,Pangrazio:2017:MDM:3097286.3097338}.} Recent studies showed that although teenagers from 14 to 18 were typically concerned about being personally identified by their personal data, they failed to perceive the potential threat of re-identification via the particular fragments they shared, e.g., images or geo-location~\cite{Pangrazio:2017:MDM:3097286.3097338}. 

Whilst there has been extensive research on \comm{teenagers'} perceptions of privacy, relatively little has been done for children aged below 11. They have often been perceived as being too young to understand privacy or exercise digital independence online~\cite{livingstone2018parentsc}.  However, developmental research has shown that children can develop a ``theory of mind" by the age of 4 \cite{colwell2016secret}, which enables children to recognise the differences between concepts in their minds and those in others, and hence to grasp complicated concepts like ``secrecy''~\cite{colwell2016secret} or ``deception''~\cite{chandler1989small}. Contrary to common expectations, children value their privacy because this enables them to enjoy their experience online \cite{Silva:2017:PCT:3091478.3091479, kumar2018cscw}, such as socialising with their friends and families or experimenting with new games. Existing literature provided us with us with useful insights into children's perception of risks \cite{zhang2016nosy, kumar2018cscw}, however, they they do not tell us how children make these judgements - or whether children can in fact identify a threat and its origination.


\subsection{Managing Children's Privacy Online}
Tools developed for managing children's privacy on mobile platforms \comm{usually comprise} features that monitor and restrict children's online activities~\cite{wisniewski2017parental,livingstone2018parentsa,ofcom2017}. Children often find these tools overly restrictive and invasive of their personal privacy \cite{Ghosh:2018:SVS:3173574.3173698,wisniewski2017parental}. Co-design studies with children under 12 show that they prefer technologies that facilitate their risk coping skill development, promote communication and interaction with their parents, and emphasise restrictions around monitoring~\cite{mcnally2018co}. However, such tools are still scarce. 

Several recent studies have recognised the importance of supporting children's learning through approaches like interactive storytelling~\cite{Zhang-Kennedy:2016:TIE:2930674.2935984}, game playing~\cite{maqsood2018day} or co-learning with parents~\cite{hashish2014involving}. They have shown the effectiveness of increasing children's awareness of related online safety issues, such as online personal identity or content appropriateness. This demonstrates that a knowledge scaffolding approach to  a child's means of dealing with privacy risk coping could provide a useful addition to safeguarding their cybersafety.


\subsection{Developmental Stages of Privacy Concepts}

Children's ability to recognise privacy risks may be intrinsically limited by their developmental stage. Children aged 3-5 start to build up friendships; however, at this stage, family interactions are dominant, and many of their online activities are still parent-guided \cite{digital2017}, peer pressure is less of an influence~\cite{ann2000developmental}. Children from 6 to 9, \comm{however}, start to learn about the complexity of relationships and feel the need to fit in to peer social groups~\cite{ann2000developmental}. They are also more involved in online activities and enjoy playing games with their friends~\cite{digital2017}. This social interaction with peers makes them more aware of interpersonal privacy risks, but less of other privacy risks \cite{digital2017}. So while they often care deeply about their personal information being shared with their peers, parents, and others online, they remain unaware of other actors, including platforms, app designers, malicious actors, and others operating in digital ecosystems~\cite{livingstone2018childrenc,Pangrazio:2017:MDM:3097286.3097338}. 

Vygotsky's Zone of Proximal Development (ZPD) is a theory that relates the difference between what learners can do independently to what can be achieved by through guidance by a skilled partner~\cite{chaiklin2003zone}. It has been applied to assess the effectiveness of teaching and learning~\cite{miller2010theories}, to identify key barriers in learning by understanding knowledge gaps~\cite{daniels2005introduction}, and in the design of better intelligent tutoring systems (ITS)~\cite{quintana2004scaffolding}. \comm{Inspired by ZPD, we focus on identifying children's misconceptions of privacy risks and highlighting areas of knowledge that could be developed through future active scaffolding. } 
